Machine-learning decoders for fusion-based quantum computing in real time

Fault-tolerant quantum computation requires decoders that combine accuracy, throughput, low latency, and scalability to large numbers of physical qubits. In photonic fusion-based architectures, erasures from photon loss and probabilistic fusion measurements are a dominant error mechanism, motivating decoders that remain accurate at high erasure rates. We introduce PRISM, a transformer-based machine-learning decoder designed to exploit the known locations of erasures in protocols subject to both Pauli and erasure errors. We benchmark PRISM across a wide range of fault-tolerant protocols based on surface codes, color codes, and quantum low-density parity-check codes, with distances up to 24. Across these benchmarks, PRISM matches the logical error rates of integer-programming-based decoders while being significantly faster, including at error rates up to 50% of threshold. We further optimize the decoder and its real-time hardware implementation to reduce latency while maintaining accuracy. Our optimized implementation on an AMD VP1902 FPGA can decode logical blocks of distance 8 in both space and time, demonstrating a latency of 6.59 microseconds and an amortized decoding time of 1.56 microseconds per logical block is possible. These results show that machine-learning decoding can provide accurate, low-latency inference for erasure-dominated fault-tolerant quantum architectures.

==> preamble/architecture_columns.tex <==
\makeatletter
\newbox\archCols@holdpg
\newcount\archCols@colnumber
\def\archCols@specialoutput{%
    \ifnum\outputpenalty<-\@Miii
        \ifnum\outputpenalty<-\@MM\deadcycles\z@\fi
        \global\setbox\@holdpg\vbox{\unvbox\@cclv}%
    \else
        \dispatch@output
    \fi
}
\newsavebox{\archCols@diagram}
\newenvironment{architecturecolumns}[2][0.7]{%
    \begingroup
    \par\medskip
    \sbox{\archCols@diagram}{\includetikz{#2}}%
    \Needspace{\dimexpr\ht\archCols@diagram+\dp\archCols@diagram+2\baselineskip\relax}%
    \def\@makecol{\@makecolumn\true@sw}
    \def\set@adj@colht##1{##1\@colht}
    \let\@specialoutput\archCols@specialoutput
    \let\@holdpg\archCols@holdpg
    \let\col@number\archCols@colnumber
    \let\output\primitive@output
    \let\archCols@marginnote\@mn@@marginnote
    \columnratio{#1}%
    \begin{paracol}{2}%
    \let\@mn@@marginnote\archCols@marginnote
}{%
    \switchcolumn
    {\centering\adjustbox{max width=\linewidth}{\usebox{\archCols@diagram}}\par}%
    \end{paracol}%
    \endgroup
}
\makeatother


==> tikz/from_data/decoder_performance_plots.tex <==
\tikzfilename{decoder_performance_plots}%
\begin{tikzpicture}
	\begin{groupplot}[csv loglog,xmode=log,ymode=log,ymin=1e-18,ymax=0.1,group style={group size=3 by 2,horizontal sep=1ex,vertical sep=20mm,y descriptions at=all}]
		\nextgroupplot[title={\textbf{(a)}\quad Six-ring},protocol axis/six_ring/.try]
		\addplot+[distance8,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/six_ring/8/ml.csv};
		\addplot[distance8,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/six_ring/8/ml.fit.csv};
		\addplot+[distance8,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/six_ring/8/benchmark.csv};
		\addplot[distance8,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/six_ring/8/benchmark.fit.csv};
		\addplot+[distance12,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/six_ring/12/ml.csv};
		\addplot[distance12,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/six_ring/12/ml.fit.csv};
		\addplot+[distance12,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/six_ring/12/benchmark.csv};
		\addplot[distance12,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/six_ring/12/benchmark.fit.csv};
		\addplot+[distance16,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/six_ring/16/ml.csv};
		\addplot+[distance16,only marks,mark=triangle*,mark options={rotate=180},
			forget plot,unbounded coords=discard]
		table[col sep=comma,x=x,
				y expr={\thisrow{num_logical_errors}==0 ? \thisrow{ler_upper} : nan}] {data/protocols/six_ring/16/ml.csv};
		\addplot[distance16,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/six_ring/16/ml.fit.csv};
		\addplot+[distance16,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/six_ring/16/benchmark.csv};
		\addplot[distance16,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/six_ring/16/benchmark.fit.csv};
		\node[anchor=south east,font=\scriptsize,fill=white,inner sep=2pt,align=left,
			benchmark decoder label/.try] at (rel axis cs:0.98,0.02)
		{Benchmark (MWPM)};
		\nextgroupplot[title={\textbf{(b)}\quad Linked loopy diamond},yticklabels={},ylabel={},legend columns=3,legend to name=decoderlegend,protocol axis/linked_loopy_diamond/.try]
		\addplot+[distance8,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/linked_loopy_diamond/8/ml.csv};
		\addplot[distance8,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/linked_loopy_diamond/8/ml.fit.csv};
		\addplot+[distance8,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/linked_loopy_diamond/8/benchmark.csv};
		\addplot[distance8,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/linked_loopy_diamond/8/benchmark.fit.csv};
		\addplot+[distance16,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/linked_loopy_diamond/16/ml.csv};
		\addplot[distance16,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/linked_loopy_diamond/16/ml.fit.csv};
		\addplot+[distance16,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/linked_loopy_diamond/16/benchmark.csv};
		\addplot[distance16,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/linked_loopy_diamond/16/benchmark.fit.csv};
		\addplot+[distance24,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/linked_loopy_diamond/24/ml.csv};
		\addplot+[distance24,only marks,mark=triangle*,mark options={rotate=180},
			forget plot,unbounded coords=discard]
		table[col sep=comma,x=x,
				y expr={\thisrow{num_logical_errors}==0 ? \thisrow{ler_upper} : nan}] {data/protocols/linked_loopy_diamond/24/ml.csv};
		\addplot[distance24,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/linked_loopy_diamond/24/ml.fit.csv};
		\addplot+[distance24,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/linked_loopy_diamond/24/benchmark.csv};
		\addplot[distance24,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/linked_loopy_diamond/24/benchmark.fit.csv};
		\node[anchor=south east,font=\scriptsize,fill=white,inner sep=2pt,align=left,
			benchmark decoder label/.try] at (rel axis cs:0.98,0.02)
		{Benchmark (BP+ILP)};
		\addlegendimage{empty legend}
		\addlegendentry{$\Dist=6$}
		\addlegendimage{distance6,solid,mark=o}
		\addlegendentry{ML}
		\addlegendimage{distance6,dashed,mark=x}
		\addlegendentry{Benchmark}
		\addlegendimage{empty legend}
		\addlegendentry{$\Dist=8$}
		\addlegendimage{distance8,solid,mark=o}
		\addlegendentry{ML}
		\addlegendimage{distance8,dashed,mark=x}
		\addlegendentry{Benchmark}
		\addlegendimage{empty legend}
		\addlegendentry{$\Dist=12$}
		\addlegendimage{distance12,solid,mark=o}
		\addlegendentry{ML}
		\addlegendimage{distance12,dashed,mark=x}
		\addlegendentry{Benchmark}
		\addlegendimage{empty legend}
		\addlegendentry{$\Dist=16$}
		\addlegendimage{distance16,solid,mark=o}
		\addlegendentry{ML}
		\addlegendimage{distance16,dashed,mark=x}
		\addlegendentry{Benchmark}
		\addlegendimage{empty legend}
		\addlegendentry{$\Dist=24$}
		\addlegendimage{distance24,solid,mark=o}
		\addlegendentry{ML}
		\addlegendimage{distance24,dashed,mark=x}
		\addlegendentry{Benchmark}
		\nextgroupplot[title={\textbf{(c)}\quad Color code},yticklabel pos=right,ylabel={},protocol axis/color_code/.try]
		\addplot+[distance8,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/color_code/8/ml.csv};
		\addplot[distance8,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/color_code/8/ml.fit.csv};
		\addplot+[distance8,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/color_code/8/benchmark.csv};
		\addplot[distance8,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/color_code/8/benchmark.fit.csv};
		\addplot+[distance16,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/color_code/16/ml.csv};
		\addplot+[distance16,only marks,mark=triangle*,mark options={rotate=180},
			forget plot,unbounded coords=discard]
		table[col sep=comma,x=x,
				y expr={\thisrow{num_logical_errors}==0 ? \thisrow{ler_upper} : nan}] {data/protocols/color_code/16/ml.csv};
		\addplot[distance16,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/color_code/16/ml.fit.csv};
		\addplot+[distance16,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/color_code/16/benchmark.csv};
		\addplot[distance16,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/color_code/16/benchmark.fit.csv};
		\addplot+[distance24,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/color_code/24/ml.csv};
		\addplot+[distance24,only marks,mark=triangle*,mark options={rotate=180},
			forget plot,unbounded coords=discard]
		table[col sep=comma,x=x,
				y expr={\thisrow{num_logical_errors}==0 ? \thisrow{ler_upper} : nan}] {data/protocols/color_code/24/ml.csv};
		\addplot[distance24,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/color_code/24/ml.fit.csv};
		\node[anchor=south east,font=\scriptsize,fill=white,inner sep=2pt,align=left,
			benchmark decoder label/.try] at (rel axis cs:0.98,0.02)
		{Benchmark (BP+ILP)};
		\nextgroupplot[title={\textbf{(d)}\quad Bivariate bicycle},protocol axis/bivariate_bicycle/.try]
		\addplot+[distance6,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/bivariate_bicycle/6/ml.csv};
		\addplot[distance6,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/bivariate_bicycle/6/ml.fit.csv};
		\addplot+[distance6,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/bivariate_bicycle/6/benchmark.csv};
		\addplot[distance6,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/bivariate_bicycle/6/benchmark.fit.csv};
		\addplot+[distance12,only marks,mark=o,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/bivariate_bicycle/12/ml.csv};
		\addplot[distance12,solid,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/bivariate_bicycle/12/ml.fit.csv};
		\addplot+[distance12,only marks,mark=x,forget plot,unbounded coords=discard,
			error bars/.cd,y dir=both,y explicit]
		table[col sep=comma,x=x,y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
				y error minus=ler_error_minus,y error plus=ler_error_plus] {data/protocols/bivariate_bicycle/12/benchmark.csv};
		\addplot[distance12,dashed,thick,no marks,forget plot]
		table[col sep=comma,x=x,y=y] {data/protocols/bivariate_bicycle/12/benchmark.fit.csv};
		\node[anchor=south east,font=\scriptsize,fill=white,inner sep=2pt,align=left,
			benchmark decoder label/.try] at (rel axis cs:0.98,0.02)
		{Benchmark (BP+OSD)};
	\end{groupplot}
	\path (group c2r1.east) -- coordinate[midway] (decoderLegendCenter) (group c3r1.west);
	\node[anchor=north,inner sep=0pt]
	at (decoderLegendCenter |- group c1r2.north)
	{\pgfplotslegendfromname{decoderlegend}};
\end{tikzpicture}


==> tikz/from_data/kernel_benchmarks_plots.tex <==
\tikzfilename{kernel_benchmarks_plots}%
\unskip
\begingroup
\providecommand{\blockBenchmarkDataDir}{data/architecture}%
\pgfplotstableread[col sep=comma]{\blockBenchmarkDataDir/block_timing.csv}\blockBenchmarkTimingTable
\def\blockBenchmarkTicks{}%
\pgfplotstableforeachcolumnelement{distance}\of\blockBenchmarkTimingTable\as\blockBenchmarkDistance{%
    \ifx\blockBenchmarkTicks\empty
        \edef\blockBenchmarkTicks{\blockBenchmarkDistance}%
    \else
        \edef\blockBenchmarkTicks{\blockBenchmarkTicks,\blockBenchmarkDistance}%
    \fi
}%
\begin{tikzpicture}
    \begin{groupplot}[
        group style={group size=2 by 1, horizontal sep=0.05\linewidth},
        width=0.38\linewidth, height=0.29\linewidth, scale only axis,
        ymode=log,
        xlabel={Protocol distance $\Dist$},
        xtick/.expanded={\blockBenchmarkTicks},
        axis lines=box,
        tick align=outside, tick pos=left,
        tick label style={font=\small}, label style={font=\small},
        every axis title shift=0pt,
        title style={at={(0,1.04)}, anchor=south west, inner sep=0pt},
        grid=both,
        major grid style={gray!30},
        minor grid style={gray!12},
        xticklabel={\num[evaluate-expression]{round(\tick,0)}},
        legend style={at={(0.02,0.98)}, anchor=north west,
            draw=none, fill=white, fill opacity=0.8, font=\scriptsize, cells={anchor=west}},
        unbounded coords=discard,
    ]
        \nextgroupplot[
            title={\textbf{(a)}},
            ylabel={Mean training-step time (\unit{\milli\second})},
            ytickten={0,1,...,3}
        ]
        \addplot[color=blockBlue, only marks, forget plot, mark=*, thick,
            error bars/.cd, y dir=both, y explicit]
            table[col sep=comma, x=distance, y=triton_attention_ms,
                y error=triton_attention_ci95_ms]
                {\blockBenchmarkDataDir/block_timing.csv};
        \addplot[color=blockBlue, thick, no marks, forget plot]
            table[col sep=comma, x=distance, y=triton_attention_ms]
                {\blockBenchmarkDataDir/block_fits.csv};
        \addlegendimage{color=blockBlue, mark=*, thick}
        \addlegendentry{Sparse attention, Triton kernel}
        \addplot[color=blockOrange, only marks, forget plot, mark=square*, thick,
            error bars/.cd, y dir=both, y explicit]
            table[col sep=comma, x=distance, y=sdpa_attention_ms,
                y error=sdpa_attention_ci95_ms]
                {\blockBenchmarkDataDir/block_timing.csv};
        \addplot[color=blockOrange, thick, no marks, forget plot]
            table[col sep=comma, x=distance, y=sdpa_attention_ms]
                {\blockBenchmarkDataDir/block_fits.csv};
        \addlegendimage{color=blockOrange, mark=square*, thick}
        \addlegendentry{Sparse attention, gather + SDPA}
        \addplot[color=blockGreen, only marks, forget plot, mark=triangle*, thick,
            error bars/.cd, y dir=both, y explicit]
            table[col sep=comma, x=distance, y=feedforward_ms,
                y error=feedforward_ci95_ms]
                {\blockBenchmarkDataDir/block_timing.csv};
        \addplot[color=blockGreen, thick, no marks, forget plot]
            table[col sep=comma, x=distance, y=feedforward_ms]
                {\blockBenchmarkDataDir/block_fits.csv};
        \addlegendimage{color=blockGreen, mark=triangle*, thick}
        \addlegendentry{Feed-forward blocks}
%
        \nextgroupplot[
            title={\textbf{(b)}},
            ylabel={Peak allocated GPU memory (\unit{\gibi\byte})},
            ytick pos=right,
            yticklabel pos=right,
            ylabel near ticks,
        ]
        \addplot[color=blockBlue, only marks, forget plot, mark=*, thick]
            table[col sep=comma, x=distance, y=triton_attention_gib]
                {\blockBenchmarkDataDir/block_memory.csv};
        \addplot[color=blockBlue, thick, no marks, forget plot]
            table[col sep=comma, x=distance, y=triton_attention_gib]
                {\blockBenchmarkDataDir/block_fits.csv};
        \addplot[color=blockOrange, only marks, forget plot, mark=square*, thick]
            table[col sep=comma, x=distance, y=sdpa_attention_gib]
                {\blockBenchmarkDataDir/block_memory.csv};
        \addplot[color=blockOrange, thick, no marks, forget plot]
            table[col sep=comma, x=distance, y=sdpa_attention_gib]
                {\blockBenchmarkDataDir/block_fits.csv};
        \addplot[color=blockGreen, only marks, forget plot, mark=triangle*, thick]
            table[col sep=comma, x=distance, y=feedforward_gib]
                {\blockBenchmarkDataDir/block_memory.csv};
        \addplot[color=blockGreen, thick, no marks, forget plot]
            table[col sep=comma, x=distance, y=feedforward_gib]
                {\blockBenchmarkDataDir/block_fits.csv};
    \end{groupplot}
\end{tikzpicture}%
\endgroup


==> tikz/from_data/qat/qat_quantizers.tex <==
\tikzfilename{qat_quantizers}%
\begingroup
\providecommand{\qatQuantizerDataFile}{data/qat/quantizer_steps.csv}%
\pgfplotstableread[col sep=comma,text indicator="]{\qatQuantizerDataFile}\qatQuantizerData

\pgfplotsset{
    qat quantizer/.style={
        width=0.19\linewidth,height=0.19\linewidth,scale only axis,
        xlabel={input / $s$},
        axis lines=box,
        tick align=outside,tick pos=left,
        tick label style={font=\scriptsize},
        label style={font=\small},
        title style={font=\scriptsize,align=left,at={(0,1.02)},
            anchor=south west,inner sep=0pt},
        every axis title shift=0pt,
        ymajorgrids,major grid style={gray!25},
        scaled ticks=false,
        unbounded coords=discard,
        axis line style={black},
    },
    qat quantizer/a/.style={
        title={\textbf{(a)} Weights\\ternary},
        ylabel={output / $s$},ymin=-1.8,ymax=1.8,
        xtick={-2,-1,0,1,2},ytick={-1,0,1},
    },
    qat quantizer/b/.style={
        title={\textbf{(b)} Activations\\signed 2-bit},
        ymin=-2.8,ymax=1.8,xtick={-2,0,2},ytick={-2,-1,0,1},
    },
    qat quantizer/c/.style={
        title={\textbf{(c)} After ReLU\\unsigned 2-bit},
        ymin=-0.8,ymax=3.8,xtick={0,2,4},ytick={0,1,2,3},
    },
    qat quantizer/d/.style={
        title={\textbf{(d)} Min-sum values\\1 sign + 2 magnitude bits},
        ymin=-4.3,ymax=4.3,xtick={-4,-2,0,2,4},ytick={-4,-2,0,2,4},
    },
}
\NewDocumentCommand{\makeqatquantizerpanel}{m}{%
    \def\qatPanel{#1}%
    % Read the displayed input domain and STE interval from this panel.
    \def\qatXmin{}%
    \pgfplotstableforeachcolumnelement{panel}\of\qatQuantizerData\as\qatRowPanel{%
        \ifx\qatRowPanel\qatPanel
            \ifx\qatXmin\empty
                \pgfplotstablegetelem{\pgfplotstablerow}{x_from}\of\qatQuantizerData
                \edef\qatXmin{\pgfplotsretval}%
                \pgfplotstablegetelem{\pgfplotstablerow}{ste_range_lo}\of\qatQuantizerData
                \edef\qatSTElo{\pgfplotsretval}%
                \pgfplotstablegetelem{\pgfplotstablerow}{ste_range_hi}\of\qatQuantizerData
                \edef\qatSTEhi{\pgfplotsretval}%
            \fi
            \pgfplotstablegetelem{\pgfplotstablerow}{x_to}\of\qatQuantizerData
            \edef\qatXmax{\pgfplotsretval}%
        \fi
    }%
    %
    \edef\qatNextAxis{%
        \noexpand\nextgroupplot[qat quantizer/#1,
            xmin=\qatXmin,xmax=\qatXmax]%
        \noexpand\def\noexpand\qatPanel{#1}%
        \noexpand\def\noexpand\qatXmin{\qatXmin}%
        \noexpand\def\noexpand\qatXmax{\qatXmax}%
        \noexpand\def\noexpand\qatSTElo{\qatSTElo}%
        \noexpand\def\noexpand\qatSTEhi{\qatSTEhi}%
    }%
    \qatNextAxis
    \edef\qatYmin{\pgfkeysvalueof{/pgfplots/ymin}}%
    \edef\qatYmax{\pgfkeysvalueof{/pgfplots/ymax}}%
    % Shading denotes the straight-through-gradient interval.
    \addplot[draw=none,fill=mainPurple,fill opacity=0.08,forget plot]
        coordinates {(\qatSTElo,\qatYmin) (\qatSTEhi,\qatYmin)
            (\qatSTEhi,\qatYmax) (\qatSTElo,\qatYmax)} \closedcycle;
    % Identity reference; horizontal quantized segments are drawn below.
    \addplot[gray!60,thin,no marks,forget plot,
        domain=\qatXmin:\qatXmax,samples=2] {x};
    \pgfplotstableforeachcolumnelement{panel}\of\qatQuantizerData\as\qatRowPanel{%
        \ifx\qatRowPanel\qatPanel
            \pgfplotstablegetelem{\pgfplotstablerow}{x_from}\of\qatQuantizerData
            \edef\qatFrom{\pgfplotsretval}%
            \pgfplotstablegetelem{\pgfplotstablerow}{x_to}\of\qatQuantizerData
            \edef\qatTo{\pgfplotsretval}%
            \pgfplotstablegetelem{\pgfplotstablerow}{output}\of\qatQuantizerData
            \edef\qatOutput{\pgfplotsretval}%
            \addplot[mainPurple,very thick,no marks,forget plot]
                coordinates {(\qatFrom,\qatOutput) (\qatTo,\qatOutput)};
        \fi
    }%
}
\begin{tikzpicture}
    \begin{groupplot}[
        qat quantizer,
        group style={group size=4 by 1,horizontal sep=0.045\linewidth},
    ]
        \makeqatquantizerpanel{a}
        \makeqatquantizerpanel{b}
        \makeqatquantizerpanel{c}
        \makeqatquantizerpanel{d}
    \end{groupplot}
\end{tikzpicture}
\endgroup


==> tikz/from_data/qat/qat_summary_plots.tex <==
\tikzfilename{qat_summary_plots}%
\pgfplotsset{
    qat precision/.is choice,
    qat precision/W2A4/.style={mark=square},
    qat precision/W2A2/.style={mark=o},
    qat precision/W4A4/.style={color=brown,mark=diamond},
    qat precision/W8A8/.style={color=violet,mark=pentagon},
    qat precision/FP32/.style={color=black,mark=*,mark options={draw=black,fill=black}},
    qat precision/BF16/.style={color=mainPurple,mark=*,mark options={draw=mainPurple,fill=mainPurple}},
}

\NewDocumentCommand{\addqatplot}{m m m m O{0}}{
	\addplot+[
		dim#2,
		xshift=#5pt,
		only marks, mark=o, qat precision=#4, forget plot,
		restrict expr to domain={\thisrow{distance}}{#1:#1},
		restrict expr to domain={\thisrow{model_dim}}{#2:#2},
		restrict expr to domain={\thisrow{x}}{#3:#3},
		x filter/.append code={%
			\edef\csvPrecision{\thisrow{precision}}%
			\def\wantedPrecision{#4}%
			\ifx\csvPrecision\wantedPrecision
			\else
				\def\pgfmathresult{nan}%
			\fi
		},
		unbounded coords=discard,
		error bars/.cd,
		y dir=both, y explicit
	]
	table[
			col sep=comma,
			x=parameters,
			y expr={\thisrow{num_logical_errors}>0 ? \thisrow{ler} : nan},
			y error minus=ler_error_minus,
			y error plus=ler_error_plus
		] {data/qat/qat_summary.csv};

}

\begin{tikzpicture}
	\begin{groupplot}[
			qat summary loglog,
			group style={group size=2 by 1,horizontal sep=1ex,vertical sep=45mm,y descriptions at=all}
		]
		\nextgroupplot[
			title={\textbf{(a)}\quad $x=\qty{1.25}{\percent}$},
			ymin=2e-5,
			ymax=3e-3,
			ytickten={-5,-4,...,-3},
			grid=both,
		]
		%
		\addqatplot{8}{16}{0.0125}{W2A4}
		\addqatplot{8}{32}{0.0125}{W2A2}
		\addqatplot{8}{48}{0.0125}{W2A2}
		%
		\addqatplot{8}{128}{0.0125}{W4A4}[-3]
		\addqatplot{8}{128}{0.0125}{W8A8}[0]
		\addqatplot{8}{128}{0.0125}{FP32}[3]
		%
		\addqatplot{8}{32}{0.0125}{BF16}
		%
		\nextgroupplot[
			title={\textbf{(b)}\quad $x=\qty{1.5}{\percent}$},
			yticklabel pos=right,
			ylabel={},
			legend to name=qatlegend,
			legend columns=4,
			legend cell align=left,
			ymin=2e-5,
			ymax=3e-3,
			ytickten={-5,-4,...,-3},
			grid=both,
		]
		%
		\addqatplot{8}{16}{0.015}{W2A4}
		\addqatplot{8}{32}{0.015}{W2A2}
		\addqatplot{8}{48}{0.015}{W2A2}
		%
        \addqatplot{8}{128}{0.015}{W4A4}[-3]
		\addqatplot{8}{128}{0.015}{W8A8}[0]
        \addqatplot{8}{128}{0.015}{FP32}[3]
		%
		\addqatplot{8}{32}{0.015}{BF16}
		%
		%
		\addlegendimage{dim16,only marks,mark=square}
			\addlegendentry{$\dM=16, \WA{2}{4}$}
		\addlegendimage{dim32,only marks,mark=o}
			\addlegendentry{$\dM=32, \WA{2}{2}$}
		\addlegendimage{mainPurple,only marks,mark=*}
			\addlegendentry{$\dM=32$, BF16 reference (\cref{fig:logical_error_rates:lld})}
		\addlegendimage{dim48,only marks,mark=o}
			\addlegendentry{$\dM=48, \WA{2}{2}$}
		\addlegendimage{brown,only marks,mark=diamond}
			\addlegendentry{$\dM=128, \WA{4}{4}$}
		\addlegendimage{violet,only marks,mark=pentagon}
			\addlegendentry{$\dM=128, \WA{8}{8}$}
        \addlegendimage{black,only marks,mark=*}
			\addlegendentry{$\dM=128$, FP32}
		%
	\end{groupplot}
	\node[anchor=north, yshift=-3em] at ($(group c1r1.south west)!0.5!(group c2r1.south east)$)   {\pgfplotslegendfromname{qatlegend}};
\end{tikzpicture}


==> tikz/from_data/qat/qat_training_dynamics.tex <==
\tikzfilename{qat_training_dynamics}%
\begingroup
\providecommand{\qatTrainingDataDir}{data/qat}%
\pgfplotstableread[col sep=comma,text indicator="]
    {\qatTrainingDataDir/learning_curves_bands.csv}\qatTrainingData
\ExplSyntaxOn
\cs_new_protected:Npn \qatBreakLegendLabel
  {
    \tl_set:Ne \qatGroupLabel { \exp_after:wN \use:n \qatGroupLabel }
    \tl_replace_all:Nnn \qatGroupLabel { , } { \\ }
  }
\ExplSyntaxOff
\pgfplotstableforeachcolumnelement{group}\of\qatTrainingData\as\qatGroup{%
    \pgfplotstablegetelem{\pgfplotstablerow}{group_label}\of\qatTrainingData
    \let\qatGroupLabel\pgfplotsretval
    \qatBreakLegendLabel
    \pgfplotstablegetelem{\pgfplotstablerow}{n_seeds}\of\qatTrainingData
    \expandafter\edef\csname qatTrainingLegend@\qatGroup\endcsname{%
        \unexpanded\expandafter{\qatGroupLabel}%
        \noexpand\\\pgfplotsretval\space runs}%
}
\pgfplotsset{
    qat training select/.style={
        restrict expr to domain={\thisrow{T}}{1:1},
        x filter/.append code={%
            \getthisrow{group}\qatRowGroup%
            \def\qatWantedGroup{#1}%
            \ifx\qatRowGroup\qatWantedGroup
            \else
                \def\pgfmathresult{nan}%
            \fi
        },
    },
}
\newcommand{\qatAddLegendEntry}[1]{\addlegendentry{\shortstack[l]{#1}}}
\NewDocumentCommand{\addqattrainingcurve}{m m}{%
    \addplot[name path=qatLower#1,draw=none,forget plot,qat training select={#1}]
        table[col sep=comma,x=step_k,
            y expr={max(\thisrow{min_ler},\thisrow{plot_floor})}]
            {\qatTrainingData};
    \addplot[name path=qatUpper#1,draw=none,forget plot,qat training select={#1}]
        table[col sep=comma,x=step_k,y=max_ler]
            {\qatTrainingData};
    \addplot[draw=none,fill=#2,fill opacity=0.13,forget plot]
        fill between[of=qatLower#1 and qatUpper#1];
    \addplot[#2,thick,no marks,forget plot,qat training select={#1}]
        table[col sep=comma,x=step_k,y=mean_ler]
            {\qatTrainingData};
    \addlegendimage{#2,thick,no marks}%
    \expandafter\let\expandafter\qatLegendText\csname qatTrainingLegend@#1\endcsname
    \expandafter\qatAddLegendEntry\expandafter{\qatLegendText}%
}
\begin{tikzpicture}
    \begin{axis}[
        width=0.55\linewidth,height=0.3\linewidth,scale only axis,
        xlabel={Training step $\left(\times10^3\right)$},ylabel={Logical error rate},
        ymode=log,ymin=2e-4,ymax=1.2,xmin=0,xmax=220,
        xtick={0,50,100,150,200},ytick={1e-3,1e-2,1e-1,1},
        axis lines=box,axis line style={black},
        tick align=outside,tick pos=left,
        tick label style={font=\small},label style={font=\small},
        title style={font=\small},
        grid=major,major grid style={gray!20},
        legend style={at={(1.04,1)},anchor=north west,draw=none,
            font=\scriptsize,cells={anchor=west},row sep=4pt},
        unbounded coords=discard,
    ]
        \addqattrainingcurve{fp_poly}{qatTrainBlue}
        \addqattrainingcurve{fp_minsum}{qatTrainGreen}
        \addqattrainingcurve{fp_ops}{qatTrainPurple}
        \addqattrainingcurve{qat}{qatTrainOrange}
        \addplot+[qatTrainOrange,only marks,mark=o,forget plot,
            restrict expr to domain={\thisrow{T}}{1:1},
            error bars/.cd,y dir=both,y explicit]
            table[col sep=comma,x=x_plot_step_k,y=ler,
                y error minus=ler_error_minus,y error plus=ler_error_plus]
                {\qatTrainingDataDir/final_qat_points.csv};
    \end{axis}
\end{tikzpicture}
\endgroup


==> tikz/from_data/qat/qat_width_scan.tex <==
\tikzfilename{qat_width_scan}%
\begingroup
\providecommand{\qatWidthDataDir}{data/qat}%
\pgfplotsset{
    qat width/.style={
        width=0.42\linewidth,height=0.25\linewidth,scale only axis,
        xlabel={Model dimension $\dM$},ylabel={Logical error rate},
        ymode=log,ymin=3e-4,ymax=2e-2,
        xmin=14,xmax=51,xtick={16,24,32,40,48},
        ytick={1e-3,1e-2},
        axis lines=box,axis line style={black},
        tick align=outside,tick pos=left,
        tick label style={font=\small},label style={font=\small},
        title style={font=\small,at={(0,1.03)},anchor=south west,inner sep=0pt},
        every axis title shift=0pt,
        grid=major,major grid style={gray!20},
        legend style={at={(0.5,-0.2)},anchor=north,draw=none,
            font=\scriptsize,cells={anchor=west},row sep=1pt},
        unbounded coords=discard,
    },
    qat width select/.style 2 args={
        x filter/.append code={%
            \edef\qatRowPanel{\thisrow{panel}}%
            \def\qatWantedPanel{#1}%
            \ifx\qatRowPanel\qatWantedPanel
            \else
                \def\pgfmathresult{nan}%
            \fi
            \edef\qatRowSeries{\thisrow{series}}%
            \def\qatWantedSeries{#2}%
            \ifx\qatRowSeries\qatWantedSeries
            \else
                \def\pgfmathresult{nan}%
            \fi
        },
    },
}
\NewDocumentCommand{\addqatwidthseries}{m m m m m O{solid}}{%
    \addplot[#3,#6,thick,no marks,forget plot,qat width select={#1}{#2}]
        table[col sep=comma,x=d_model,y=geomean_ler]
            {\qatWidthDataDir/width_scan_lines.csv};
    \def\qatMarker{#4}%
    \def\qatNoMarker{none}%
    \ifx\qatMarker\qatNoMarker
    \else
        \addplot+[#3,only marks,mark=#4,forget plot,qat width select={#1}{#2},
            error bars/.cd,y dir=both,y explicit]
            table[col sep=comma,x=d_model,y=ler,
                y error minus=ler_error_minus,y error plus=ler_error_plus]
                {\qatWidthDataDir/width_scan_points.csv};
    \fi
    \addlegendimage{#3,#6,mark=#4}\addlegendentry[align=left]{#5}%
}
\begin{tikzpicture}
    \begin{groupplot}[qat width, group style={group size=2 by 1, horizontal sep=0.02\linewidth}]
        \nextgroupplot[title={\textbf{(a)}\quad\WA{2}{4}}]
        \addqatwidthseries{a}{4_2_LRx1}{qatWidthOrange}{square}     {$\text{LR}=\eta_0\times1$}
        \addqatwidthseries{a}{4_2_LRx3}{qatWidthGreen}{triangle}    {$\text{LR}=\eta_0\times3$}
        \addqatwidthseries{a}{4_2_LRx10}{qatWidthPurple}{diamond}   {$\text{LR}=\eta_0\times10$}
        \nextgroupplot[title={\textbf{(b)}\quad\WA{2}{2}},
            ylabel={},xmin=23,xmax=51,ytick pos=right,
            yticklabel pos=right,
            ylabel near ticks,]
        \addqatwidthseries{b}{W2A2_LRx10_210k}{qatWidthBlue}{o}         {$\text{LR}=\eta_0\times10$, 210k steps}
        \addqatwidthseries{b}{W2A2_LRx20_410k}{qatWidthOrange}{square}
            {$\text{LR}=\eta_0\times20$, 410k steps}
        \addqatwidthseries{b}{reference_W2A4_N_M_4_2_LRx10}{black!55}{none}
            {$\text{LR}=\eta_0\times10$ (\WA{2}{4} reference)}[dashed]
    \end{groupplot}
\end{tikzpicture}
\endgroup


==> tikz/from_data/training_curriculum.tex <==
\tikzfilename{training_curriculum}%
\unskip%
\begingroup%
\providecommand{\curriculumProtocol}{LLD}%
\edef\selectedProtocol{\curriculumProtocol}%
\pgfplotstableread[col sep=comma]{data/training/training_curriculum.csv}\curriculumTable%
\ifdefined\curriculumDistance%
\else%
    \def\curriculumDistance{0}%
    \pgfplotstableforeachcolumnelement{protocol}\of\curriculumTable\as\protocol{%
        \ifx\protocol\selectedProtocol%
            \pgfplotstablegetelem{\pgfplotstablerow}{distance}\of\curriculumTable%
            \ifnum\pgfplotsretval>\curriculumDistance\relax%
                \let\curriculumDistance\pgfplotsretval%
            \fi%
        \fi%
    }%
\fi%
\def\curriculumPointCount{0}%
\pgfplotsinvokeforeach{lr_factor,weight_decay_factor,dropout_factor,error_temperature}{%
    \expandafter\def\csname curriculum@#1\endcsname{}%
}%
\def\appendCurriculumValue#1{%
    \pgfplotstablegetelem{\curriculumRow}{#1}\of\curriculumTable%
    \expandafter\let\csname curriculumValue@#1@\curriculumPointCount\endcsname\pgfplotsretval%
    \expandafter\edef\csname curriculum@#1\endcsname{%
        \csname curriculum@#1\endcsname (\curriculumEpoch,\pgfplotsretval)}%
}%
\pgfplotstableforeachcolumnelement{protocol}\of\curriculumTable\as\protocol{%
    \ifx\protocol\selectedProtocol%
        \pgfplotstablegetelem{\pgfplotstablerow}{distance}\of\curriculumTable%
        \ifnum\pgfplotsretval=\curriculumDistance\relax%
            \edef\curriculumRow{\pgfplotstablerow}%
            \pgfplotstablegetelem{\curriculumRow}{epoch}\of\curriculumTable%
            \let\curriculumEpoch\pgfplotsretval%
            \expandafter\edef\csname curriculumEpoch@\curriculumPointCount\endcsname{\curriculumEpoch}%
            \pgfplotstablegetelem{\curriculumRow}{steps}\of\curriculumTable%
            \let\curriculumTotalSteps\pgfplotsretval%
            \appendCurriculumValue{lr_factor}%
            \appendCurriculumValue{weight_decay_factor}%
            \appendCurriculumValue{dropout_factor}%
            \appendCurriculumValue{error_temperature}%
            \edef\curriculumPointCount{\number\numexpr\curriculumPointCount+1\relax}%
        \fi%
    \fi%
}%
\ifnum\curriculumPointCount<2\relax%
    \PackageError{training_curriculum_csv}{No complete curriculum for%
        \curriculumProtocol, distance \curriculumDistance}{Check the selected protocol and distance.}%
\fi%
\edef\curriculumLastPoint{\number\numexpr\curriculumPointCount-1\relax}%
\edef\curriculumLastEpoch{\csname curriculumEpoch@\curriculumLastPoint\endcsname}%
\edef\curriculumStepsPerEpoch{\number\numexpr\curriculumTotalSteps/\curriculumLastEpoch\relax}%
\begin{tikzpicture}[
    learning rate/.style={draw=curriculumBlue, line width=2.1pt},
    weight decay/.style={draw=curriculumOrange, line width=1.5pt},
    dropout/.style={draw=curriculumGreen, line width=0.9pt, dash pattern=on 3pt off 1.5pt},
    error temperature/.style={draw=curriculumPink, line width=0.9pt,
        dash pattern=on 3pt off 1.5pt on 0.6pt off 1.5pt},
]
    \begin{axis}[
        width=0.667\linewidth, height=0.32\linewidth,
        xmin=0, xmax=\curriculumLastEpoch, ymin=-0.04, ymax=1.04,
        enlargelimits=false,
        xlabel={Epoch}, ylabel={Curriculum value},
        label style={font=\small},
        axis lines=box,
        axis line style={black},
        xtick distance=20, ytick={0,0.2,...,1},
        tick align=outside, tick pos=left,
        tick style={black},
        tick label style={font=\small},
        yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=1,
            /pgf/number format/fixed zerofill},
        clip=true, clip mode=global, clip marker paths=true,
        legend columns=4,
        legend style={
            at={(0.5,-0.25)},
            anchor=north,
            draw=black!10,
            font=\scriptsize,
            name=curriculumLegend,
        },
    ]
        \pgfplotsinvokeforeach{1,...,\curriculumLastPoint}{%
            \edef\previousPoint{\number\numexpr#1-1\relax}%
            \def\phaseColour{curriculumRamp}%
            \pgfmathparse{%
                (\csname curriculumValue@weight_decay_factor@#1\endcsname <
                    \csname curriculumValue@weight_decay_factor@\previousPoint\endcsname) ||
                (\csname curriculumValue@dropout_factor@#1\endcsname <
                    \csname curriculumValue@dropout_factor@\previousPoint\endcsname)}%
            \ifdim\pgfmathresult pt>0pt
                \def\phaseColour{curriculumAnneal}%
            \fi
            \pgfmathparse{\csname curriculumValue@lr_factor@#1\endcsname -
                \csname curriculumValue@lr_factor@\previousPoint\endcsname}%
            \ifdim\pgfmathresult pt>0pt
                \def\phaseColour{curriculumWarmup}%
            \else
                \ifdim\pgfmathresult pt<0pt
                    \def\phaseColour{curriculumFinal}%
                \fi
            \fi
            \edef\drawCurriculumPhase{%
                \noexpand\fill[\phaseColour]
                    (axis cs:\csname curriculumEpoch@\previousPoint\endcsname,-0.04)
                    rectangle (axis cs:\csname curriculumEpoch@#1\endcsname,1.04);}%
            \drawCurriculumPhase
        }

        \pgfplotsinvokeforeach{0,0.2,...,1}{
            \draw[white, line width=0.5pt]
                (axis cs:0,#1) -- (axis cs:\curriculumLastEpoch,#1);
        }
        \pgfplotsinvokeforeach{1,...,\number\numexpr\curriculumLastPoint-1\relax}{
            \draw[black!40, line width=0.4pt, densely dashed]
                (axis cs:\csname curriculumEpoch@#1\endcsname,-0.04) --
                (axis cs:\csname curriculumEpoch@#1\endcsname,1.04);
        }

        \addplot[learning rate, no marks]
            coordinates {\csname curriculum@lr_factor\endcsname};
        \addlegendentry{Learning-rate factor}
        \addplot[weight decay, no marks]
            coordinates {\csname curriculum@weight_decay_factor\endcsname};
        \addlegendentry{Weight-decay factor}
        \addplot[dropout, no marks]
            coordinates {\csname curriculum@dropout_factor\endcsname};
        \addlegendentry{Dropout factor}
        \addplot[error temperature, no marks]
            coordinates {\csname curriculum@error_temperature\endcsname};
        \addlegendentry{Error temperature}
    \end{axis}

\end{tikzpicture}%
\endgroup


==> tikz/fusion_networks/6ring.tex <==
\tikzfilename{6ring}%
\unskip%
\begingroup%
\begin{tikzpicture}[
    x=0.5bp, y=-0.5bp,
    edge/.style={draw=black, line width=2.25bp, line cap=round,
        preaction={draw=white, line width=6.75bp, line cap=round}},
    vertex/.style={draw=black, fill=fusionVertex, line width=2.25bp},
]
    \path[use as bounding box] (0,0) rectangle (1272,1237);

    \foreach \i/\x/\y in {
        0/658.0/71.8,1/369.1/179.5,2/927.0/179.6,
        3/96.5/280.5,4/631.6/280.7,5/1178.0/293.0,
        6/344.0/385.5,7/892.5/393.7,8/658.0/406.5,
        9/599.0/497.6,10/370.6/507.0,11/927.1/521.2,
        12/96.5/598.7,13/631.4/618.2,14/1177.8/628.2,
        15/344.0/707.3,16/890.7/726.4,17/658.0/731.7,
        18/599.2/822.8,19/369.5/825.2,20/925.3/838.0,
        21/96.0/911.0,22/630.4/934.8,23/1177.4/943.9,
        24/341.1/1028.9,25/889.5/1043.7,26/597.3/1145.4%
    } {
        \coordinate (v\i) at (\x,\y);
    }

    \foreach \a/\b in {
        8/17,17/19,17/20,0/8,8/10,8/11,
        10/19,11/20,19/21,19/22,20/22,20/23,
        0/1,0/2,1/10,2/11,10/12,10/13,
        11/13,12/21,11/14,13/22,21/24,14/23,
        22/24,22/25,23/25,1/3,1/4,2/4,
        3/12,2/5,4/13,12/15,5/14,13/15,
        13/16,14/16,15/24,16/25,24/26,25/26,
        3/6,4/6,4/7,5/7,6/15,7/16,
        15/18,16/18,18/26,6/9,7/9,9/18%
    } {
        \draw[edge] (v\a) -- (v\b);
    }

    \foreach \i in {0,...,26} {
        \filldraw[vertex] (v\i) circle[radius=17.5];
    }
\end{tikzpicture}%
\endgroup



==> tikz/fusion_networks/cc8.tex <==
\tikzfilename{cc8}%
\unskip%
\begingroup%
\begin{tikzpicture}[
    x=0.5bp, y=-0.5bp,
    edge/.style={draw=black, line width=1.5bp, line cap=round,
        preaction={draw=white, line width=4.5bp, line cap=round}},
    vertex/.style={draw=black, fill=fusionVertex, line width=1.5bp},
]
    \path[use as bounding box] (0,0) rectangle (1330,1296);

    \foreach \i/\x/\y in {
        0/967.5/43.5,1/1055.5/207.5,2/279.5/231.5,
        3/719.5/301.5,4/1263.5/301.5,5/373.5/395.5,
        6/921.5/401.5,7/39.5/493.5,8/577.5/495.5,
        9/1021.5/563.5,10/467.5/571.5,11/235.5/587.5,
        12/1109.5/733.5,13/327.5/761.5,14/877.5/763.5,
        15/777.5/829.5,16/1311.5/833.5,17/977.5/927.5,
        18/423.5/929.5,19/87.5/1019.5,20/623.5/1019.5,
        21/1071.5/1085.5,22/283.5/1113.5,23/379.5/1277.5%
    } {
        \coordinate (v\i) at (\x,\y);
    }

    \foreach \a/\b in {
        12/21,12/15,12/16,15/21,9/12,10/15,
        16/21,9/15,1/9,15/18,1/3,10/18,
        3/10,17/21,9/16,15/17,1/4,3/9,
        0/1,5/10,16/17,9/17,4/9,18/23,
        0/3,18/19,3/5,6/9,0/4,18/20,
        3/6,19/23,13/18,17/20,4/6,20/23,
        0/6,13/19,5/13,5/7,14/17,22/23,
        13/20,19/22,5/8,7/13,2/5,14/20,
        6/14,20/22,6/8,13/22,8/13,2/7,
        8/14,11/13,2/8,7/11,8/11,2/11%
    } {
        \draw[edge] (v\a) -- (v\b);
    }

    \foreach \i in {0,...,23} {
        \filldraw[vertex] (v\i) circle[radius=14];
    }
\end{tikzpicture}%
\endgroup



==> tikz/fusion_networks/lld.tex <==
\tikzfilename{lld}%
\unskip%
\begingroup%
\begin{tikzpicture}[
    x=0.5bp, y=-0.5bp,
    edge/.style={draw=black, line width=1bp, line cap=round},
    edge halo/.style={draw=white, line width=3bp, line cap=round},
    vertex/.style={draw=black, fill=fusionVertex, line width=1bp},
]
    \path[use as bounding box] (0,0) rectangle (665,648);

    \foreach \i/\x/\y in {
        0/483.4/21.3,1/527.8/103.0,2/140.0/115.1,
        3/359.8/150.5,4/631.4/150.6,5/186.2/198.0,
        6/460.2/200.2,7/19.5/246.6,8/288.0/247.9,
        9/511.1/282.0,10/233.5/285.5,11/117.9/293.0,
        12/554.1/367.0,13/164.2/380.2,14/438.2/381.4,
        15/388.4/414.5,16/655.8/416.8,17/489.0/463.1,
        18/211.8/464.2,19/312.2/509.5,20/43.9/509.5,
        21/535.3/542.7,22/141.1/557.0,23/189.7/638.8%
    } {
        \coordinate (v\i) at (\x,\y);
    }

    \draw[edge halo] (v12) -- (v21);
    \draw[edge halo] (v12) -- (v15);
    \draw[edge halo] (v12) -- (v16);
    \draw[edge halo] (v15) -- (v21);
    \fill[fusionCheck, opacity=0.25] (v12) -- (v15) -- (v21) -- cycle;
    \draw[edge] (v12) -- (v21);
    \draw[edge] (v12) -- (v15);
    \draw[edge] (v15) -- (v21);
    \draw[edge halo] (v9) -- (v12);
    \draw[edge halo] (v10) -- (v15);
    \draw[edge] (v10) -- (v15);
    \draw[edge halo] (v16) -- (v21);
    \draw[edge halo] (v9) -- (v15);
    \draw[edge halo] (v1) -- (v9);
    \draw[edge halo] (v15) -- (v18);
    \draw[edge] (v15) -- (v18);
    \draw[edge halo] (v1) -- (v3);
    \draw[edge halo] (v10) -- (v18);
    \draw[edge] (v10) -- (v18);
    \draw[edge halo] (v3) -- (v10);
    \draw[edge halo] (v17) -- (v21);
    \draw[edge halo] (v9) -- (v16);
    \fill[fusionCheck, opacity=0.25] (v9) -- (v12) -- (v16) -- cycle;
    \draw[edge] (v12) -- (v16);
    \draw[edge] (v9) -- (v12);
    \filldraw[vertex] (v12) circle[radius=7.5];
    \draw[edge] (v9) -- (v16);
    \draw[edge halo] (v15) -- (v17);
    \draw[edge halo] (v1) -- (v4);
    \draw[edge halo] (v3) -- (v9);
    \fill[fusionCheck, opacity=0.25] (v1) -- (v3) -- (v9) -- cycle;
    \draw[edge] (v1) -- (v9);
    \draw[edge] (v1) -- (v3);
    \draw[edge] (v3) -- (v9);
    \draw[edge halo] (v0) -- (v1);
    \draw[edge halo] (v5) -- (v10);
    \draw[edge halo] (v16) -- (v17);
    \fill[fusionCheck, opacity=0.25] (v16) -- (v17) -- (v21) -- cycle;
    \draw[edge] (v16) -- (v21);
    \draw[edge] (v17) -- (v21);
    \filldraw[vertex] (v21) circle[radius=7.5];
    \draw[edge] (v16) -- (v17);
    \filldraw[vertex] (v16) circle[radius=7.5];
    \draw[edge halo] (v9) -- (v17);
    \fill[fusionCheck, opacity=0.25] (v9) -- (v15) -- (v17) -- cycle;
    \draw[edge] (v9) -- (v15);
    \draw[edge] (v15) -- (v17);
    \filldraw[vertex] (v15) circle[radius=7.5];
    \draw[edge] (v9) -- (v17);
    \draw[edge halo] (v4) -- (v9);
    \draw[edge halo] (v18) -- (v23);
    \draw[edge halo] (v0) -- (v3);
    \draw[edge halo] (v18) -- (v20);
    \draw[edge halo] (v3) -- (v5);
    \fill[fusionCheck, opacity=0.25] (v3) -- (v5) -- (v10) -- cycle;
    \draw[edge] (v3) -- (v10);
    \draw[edge] (v5) -- (v10);
    \filldraw[vertex] (v10) circle[radius=7.5];
    \draw[edge] (v3) -- (v5);
    \draw[edge halo] (v6) -- (v9);
    \draw[edge halo] (v0) -- (v4);
    \fill[fusionCheck, opacity=0.25] (v0) -- (v1) -- (v4) -- cycle;
    \draw[edge] (v1) -- (v4);
    \draw[edge] (v0) -- (v1);
    \filldraw[vertex] (v1) circle[radius=7.5];
    \draw[edge] (v0) -- (v4);
    \draw[edge halo] (v18) -- (v19);
    \draw[edge halo] (v3) -- (v6);
    \draw[edge halo] (v20) -- (v23);
    \fill[fusionCheck, opacity=0.25] (v18) -- (v20) -- (v23) -- cycle;
    \draw[edge] (v18) -- (v23);
    \draw[edge] (v18) -- (v20);
    \draw[edge] (v20) -- (v23);
    \draw[edge halo] (v13) -- (v18);
    \draw[edge halo] (v17) -- (v19);
    \draw[edge] (v17) -- (v19);
    \draw[edge halo] (v4) -- (v6);
    \fill[fusionCheck, opacity=0.25] (v4) -- (v6) -- (v9) -- cycle;
    \draw[edge] (v4) -- (v9);
    \draw[edge] (v6) -- (v9);
    \filldraw[vertex] (v9) circle[radius=7.5];
    \draw[edge] (v4) -- (v6);
    \filldraw[vertex] (v4) circle[radius=7.5];
    \draw[edge halo] (v19) -- (v23);
    \draw[edge halo] (v0) -- (v6);
    \fill[fusionCheck, opacity=0.25] (v0) -- (v3) -- (v6) -- cycle;
    \draw[edge] (v0) -- (v3);
    \draw[edge] (v3) -- (v6);
    \filldraw[vertex] (v3) circle[radius=7.5];
    \draw[edge] (v0) -- (v6);
    \filldraw[vertex] (v0) circle[radius=7.5];
    \draw[edge halo] (v13) -- (v20);
    \draw[edge halo] (v5) -- (v13);
    \draw[edge halo] (v5) -- (v7);
    \draw[edge halo] (v14) -- (v17);
    \draw[edge] (v14) -- (v17);
    \filldraw[vertex] (v17) circle[radius=7.5];
    \draw[edge halo] (v22) -- (v23);
    \draw[edge halo] (v13) -- (v19);
    \fill[fusionCheck, opacity=0.25] (v13) -- (v18) -- (v19) -- cycle;
    \draw[edge] (v18) -- (v19);
    \draw[edge] (v13) -- (v18);
    \filldraw[vertex] (v18) circle[radius=7.5];
    \draw[edge] (v13) -- (v19);
    \draw[edge halo] (v20) -- (v22);
    \draw[edge halo] (v5) -- (v8);
    \draw[edge halo] (v7) -- (v13);
    \fill[fusionCheck, opacity=0.25] (v5) -- (v7) -- (v13) -- cycle;
    \draw[edge] (v5) -- (v13);
    \draw[edge] (v5) -- (v7);
    \draw[edge] (v7) -- (v13);
    \draw[edge halo] (v2) -- (v5);
    \draw[edge halo] (v14) -- (v19);
    \draw[edge] (v14) -- (v19);
    \draw[edge halo] (v6) -- (v14);
    \draw[edge halo] (v19) -- (v22);
    \fill[fusionCheck, opacity=0.25] (v19) -- (v22) -- (v23) -- cycle;
    \draw[edge] (v19) -- (v23);
    \draw[edge] (v22) -- (v23);
    \filldraw[vertex] (v23) circle[radius=7.5];
    \draw[edge] (v19) -- (v22);
    \filldraw[vertex] (v19) circle[radius=7.5];
    \draw[edge halo] (v6) -- (v8);
    \draw[edge halo] (v13) -- (v22);
    \fill[fusionCheck, opacity=0.25] (v13) -- (v20) -- (v22) -- cycle;
    \draw[edge] (v13) -- (v20);
    \draw[edge] (v20) -- (v22);
    \filldraw[vertex] (v20) circle[radius=7.5];
    \draw[edge] (v13) -- (v22);
    \draw[edge halo] (v8) -- (v13);
    \draw[edge halo] (v2) -- (v7);
    \draw[edge halo] (v8) -- (v14);
    \fill[fusionCheck, opacity=0.25] (v6) -- (v8) -- (v14) -- cycle;
    \draw[edge] (v6) -- (v14);
    \draw[edge] (v6) -- (v8);
    \filldraw[vertex] (v6) circle[radius=7.5];
    \draw[edge] (v8) -- (v14);
    \filldraw[vertex] (v14) circle[radius=7.5];
    \filldraw[vertex] (v22) circle[radius=7.5];
    \draw[edge halo] (v11) -- (v13);
    \draw[edge halo] (v2) -- (v8);
    \fill[fusionCheck, opacity=0.25] (v2) -- (v5) -- (v8) -- cycle;
    \draw[edge] (v5) -- (v8);
    \draw[edge] (v2) -- (v5);
    \filldraw[vertex] (v5) circle[radius=7.5];
    \draw[edge] (v2) -- (v8);
    \draw[edge halo] (v7) -- (v11);
    \draw[edge halo] (v8) -- (v11);
    \fill[fusionCheck, opacity=0.25] (v8) -- (v11) -- (v13) -- cycle;
    \draw[edge] (v8) -- (v13);
    \draw[edge] (v11) -- (v13);
    \filldraw[vertex] (v13) circle[radius=7.5];
    \draw[edge] (v8) -- (v11);
    \filldraw[vertex] (v8) circle[radius=7.5];
    \draw[edge halo] (v2) -- (v11);
    \fill[fusionCheck, opacity=0.25] (v2) -- (v7) -- (v11) -- cycle;
    \draw[edge] (v2) -- (v7);
    \draw[edge] (v7) -- (v11);
    \filldraw[vertex] (v7) circle[radius=7.5];
    \draw[edge] (v2) -- (v11);
    \filldraw[vertex] (v2) circle[radius=7.5];
    \filldraw[vertex] (v11) circle[radius=7.5];
\end{tikzpicture}%
\endgroup



==> tikz/overview.tex <==
\tikzfilename{overview}%

\begin{tikzpicture}[
  font=\footnotesize,
  >={Stealth[length=3.2pt,width=2.6pt]},
  lab/.style={align=center, font=\footnotesize},
  mech/.style={circle, draw=black!60, fill=white, minimum size=2.6mm, inner sep=0pt, line width=0.45pt},
  mechE/.style={mech, path picture={\draw[ovEra, line width=0.6pt] (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.north west) -- (path picture bounding box.south east);}},
  mechP/.style={mech, fill=ovErr!75},
  chk/.style={rectangle, draw=black!60, fill=white, minimum size=2.5mm, inner sep=0pt, line width=0.45pt},
  chkF/.style={chk, fill=ovChk!85},
  edge/.style={black!45, line width=0.45pt},
  memb/.style={mech, fill=ovMem!30},
]
% ======================= (a) block =======================
\begin{scope}[shift={(0,0)}]
    \node[font=\small\bfseries, anchor=west] at (-0.35,3.35) {(a)};
    \def\c{2.3} \def\dx{0.95} \def\dy{0.62}
    % back faces
    \coordinate (A) at (0,0); \coordinate (B) at (\c,0); \coordinate (C) at (\c,\c); \coordinate (D) at (0,\c);
    \coordinate (A2) at (\dx,\dy); \coordinate (B2) at (\c+\dx,\dy); \coordinate (C2) at (\c+\dx,\c+\dy); \coordinate (D2) at (\dx,\c+\dy);
    \draw[black!35, line width=0.4pt, dashed] (A) -- (A2) -- (B2) (A2) -- (D2);
    % membrane representatives (planes at fixed depth) - translates along the depth direction
    \foreach \t/\op in {0.22/0.10, 0.5/0.28, 0.78/0.10} {
      \fill[ovMem, opacity=\op] ($(A)!\t!(A2)$) -- ($(B)!\t!(B2)$) -- ($(C)!\t!(C2)$) -- ($(D)!\t!(D2)$) -- cycle;
    }
    \foreach \t in {0.22, 0.78} {
      \draw[ovMem, dashed, line width=0.5pt] ($(A)!\t!(A2)$) -- ($(B)!\t!(B2)$) -- ($(C)!\t!(C2)$) -- ($(D)!\t!(D2)$) -- cycle;
    }
    \draw[ovMem, line width=0.7pt] ($(A)!0.5!(A2)$) -- ($(B)!0.5!(B2)$) -- ($(C)!0.5!(C2)$) -- ($(D)!0.5!(D2)$) -- cycle;
    % error chain winding along the depth direction through the membrane
    \draw[ovErr, line width=1.1pt, decorate, decoration={zigzag, segment length=4pt, amplitude=1.2pt}]
      ($(A)!0.5!(C) + (0,0)$) -- ++(\dx,\dy);
    \fill[ovErr] ($(A)!0.5!(C)$) circle (0.9pt);
    \fill[ovErr] ($(A)!0.5!(C) + (\dx,\dy)$) circle (0.9pt);
    % front cube
    \draw[black!70, line width=0.55pt] (A) -- (B) -- (C) -- (D) -- cycle;
    \draw[black!70, line width=0.55pt] (B) -- (B2) -- (C2) -- (D2) -- (D) (C) -- (C2);
    % periodic identification marks
    \foreach \p/\q in {A/B, D/C} { \draw[black!60, ->, line width=0.4pt] ($(\p)!0.42!(\q)$) -- ($(\p)!0.58!(\q)$); }
    \foreach \p/\q in {A/D, B/C} { \draw[black!60, ->>, line width=0.4pt] ($(\p)!0.42!(\q)$) -- ($(\p)!0.58!(\q)$); }
    % Matching triple-arrow marks identify periodicity in the front/back direction.
    \foreach \p/\q in {D/D2, C/C2} {
      \draw[black!60, -{Stealth[length=3.2pt,width=2.6pt]
        Stealth[length=3.2pt,width=2.6pt] Stealth[length=3.2pt,width=2.6pt]}, line width=0.4pt]
        ($(\p)!0.25!(\q)$) -- ($(\p)!0.75!(\q)$);
    }
    \node[lab, text=ovMem!90!black] at (1.9,-0.45) {membrane representatives};
    \node[lab, text=ovErr!90!black, anchor=west] at (3.35,1.55) {logical\\[-1pt]error};
    \draw[ovErr!80!black, line width=0.4pt] (3.33,1.55) -- ($(A)!0.5!(C) + (0.5*\dx,0.5*\dy) + (0.08,0)$);
    \draw[->, shift={(-0.5,0)}] (0,0)--(0,1) node [pos=1,above] {time};
\end{scope}

% ======================= (b) Tanner graph fragment =======================
\begin{scope}[shift={(5.6,0.15)}]
    \node[font=\small\bfseries, anchor=west] at (-0.35,3.2) {(b)};
    \begin{scope}[scale=4/7, shift={(1,2)}]
        \foreach \i/\x/\y in {
            1/0/0,
            2/1.72/2,
            3/1.75/-2.33,
            4/7.33/0,
            5/5.58/2,
            6/5.58/-2.33,
            7/3.665/0
        } {
            \coordinate (m\i) at (\x,\y);
        }

        \coordinate (q1) at (3.665,2.75);
        \coordinate (q2) at (4.6225,-1.165);
        \coordinate (q3) at (2.7075,-1.165);
        \coordinate (q4) at (2.7075,1);
        \coordinate (q5) at (4.6225,1);
        \coordinate (q6) at (3.665,-2.33);
        \coordinate (q7) at (.875,-1.165);
        \coordinate (q8) at (.875,1);
        \coordinate (q9) at (1.75,-.165);
        \coordinate (q10) at (6.455,-1.165);
        \coordinate (q11) at (6.455,1);
        \coordinate (q12) at (5.58,-.165);
%
        \draw (m1) -- (-.55,0) -- (-.55,2.75) -- (q1)
        -- (7.88,2.75) -- (7.88,0) -- (m4);
        \foreach \i/\a/\b in {
            2/6/7, 3/3/7, 4/2/7, 5/5/7, 6/3/6,
            7/1/3, 8/1/2, 9/2/3, 10/4/6, 11/4/5, 12/5/6} {\draw (m\a) -- (q\i) -- (m\b);}
        \foreach \i in {1,...,7} {\node[chk] at (m\i) {};}

        \foreach \i in {1,...,12} {
            \node[mech] at (q\i) {};
            }

        \foreach \i in {2,3,6} {
            \node[memb] at (q\i) {};
        }

        \foreach \i in {7,11} {
            \node[mechE] at (q\i) {};
        }

        \foreach \i in {4,5,12} {
            \node[mechP] at (q\i) {};
        }

        \foreach \i in {2,6} {
            \node[chkF] at (m\i) {};
        }
%
    \end{scope}

    \begin{scope}[shift={(-0.1,-0.72)}]
        \node[mech] at (0,0) {}; \node[lab, anchor=west, font=\scriptsize] at (0.12,0) {mechanism};
        \node[mechE] at (1.9,0) {}; \node[lab, anchor=west, font=\scriptsize] at (2.02,0) {erased};
        \node[mechP] at (3.25,0) {}; \node[lab, anchor=west, font=\scriptsize] at (3.37,0) {Pauli error};
        \node[chk] at (0,-0.4) {}; \node[lab, anchor=west, font=\scriptsize] at (0.12,-0.4) {check};
        \node[chkF] at (1.9,-0.4) {}; \node[lab, anchor=west, font=\scriptsize] at (2.02,-0.4) {flipped};
        \node[memb] at (3.25,-0.4) {}; \node[lab, anchor=west, font=\scriptsize] at (3.37,-0.4) {membrane support};
    \end{scope}
\end{scope}

% ======================= (c) decoding task =======================
\begin{scope}[shift={(11.6,0.15)}]
\node[font=\small\bfseries, anchor=west] at (-0.35,3.2) {(c)};
\node[lab, draw=black!60, rounded corners=2pt, fill=black!4, minimum width=2.4cm, minimum height=0.55cm] (inp) at (1.25,2.45) {$(\synd,\er)$};
\node[lab, draw=black!60, rounded corners=2pt, fill=ovMem!12, minimum width=2.4cm, minimum height=0.9cm] (dec) at (1.25,1.3) {decoder\\[-1pt]$p(\f_\mu\,|\,\synd,\er)$};
\node[lab, draw=black!60, rounded corners=2pt, fill=black!4, minimum width=2.4cm, minimum height=0.55cm] (outp) at (1.25,0.1) {$\hat \f_\class,\ \class=1,\dots,\nClasses$};
\draw[black!75, ->, line width=0.5pt] (inp) -- (dec);
\draw[black!75, ->, line width=0.5pt] (dec) -- (outp);
\node[lab, text=black!65, align=left, anchor=west] at (-0.2,-0.75) {\scriptsize failure if $\hat \f_\class\neq \f_\class$ for any class};
\end{scope}
\end{tikzpicture}

